Predictive Closed-Loop Remote Control over Wireless Two-Way Split Koopman Autoencoder

Real-time remote control over wireless is an important-yet-challenging application in 5G and beyond due to its mission-critical nature under limited communication resources. Current solutions hinge on not only utilizing ultra-reliable and low-latency communication (URLLC) links but also predicting future states, which may consume enormous communication resources and struggle with a short prediction time horizon. To fill this void, in this article we propose a novel two-way Koopman autoencoder (AE) approach wherein: 1) a sensing Koopman AE learns to understand the temporal state dynamics and predicts missing packets from a sensor to its remote controller; and 2) a controlling Koopman AE learns to understand the temporal action dynamics and predicts missing packets from the controller to an actuator co-located with the sensor. Specifically, each Koopman AE aims to learn the Koopman operator in the hidden layers while the encoder of the AE aims to project the non-linear dynamics onto a lifted subspace, which is reverted into the original non-linear dynamics by the decoder of the AE. The Koopman operator describes the linearized temporal dynamics, enabling long-term future prediction and coping with missing packets and closed-form optimal control in the lifted subspace. Simulation results corroborate that the proposed approach achieves a 38x lower mean squared control error at 0 dBm signal-to-noise ratio (SNR) than the non-predictive baseline.

==> Closed-Loop Koopman_Camera_Ready/Sec2_System_Model.tex <==
% \clearpage

\section{System Model}
\label{System_Model}

 \label{Wireless_Networked_Control_System_Architecture}
 Consider a closed-loop \emph{WNCS} which comprises a \emph{plant} that exhibits non-linear dynamics, a \emph{sensor} that samples the plant's state, a \emph{controller} that computes optimal control actions based on the sampled states, and an \emph{actuator} that applies the control action command on the plant received from the controller. Specifically, as illustrated in Fig.~\ref{fig_system} we assume that the sensor and actuator are co-located and share the same transceiver. On the other hand, the controller is located away from them with a computational capability to produce control action commands to ensure system stability. On this account, the controller operates remotely over wireless channels, by receiving the sensors' sampled states via the forward link and feeding back the computed optimal control action commands to the actuators via the reverse link.
 
 \subsection{Control System Architecture}
 Consider that the control system operates at a fixed \emph{control period} $\tau_o>0$ seconds to keep the plant stable over time. Hence the sensor samples the state of the plant at a fixed sampling rate $1/\tau_o$ and transmits the samples to the controller over wireless links. The $m$-th sampled state of the plant at time $t = m\tau_o$ is denoted by a $p$-dimensional vector $\mathbf{x}_{m} = [x_{m,1}\ x_{m,2}\ \cdots\ x_{m,p}] \in \mathbb{R}^{p}$. On the other hand, an optimal control action command computed at the controller based on the $m$-th sample $\mathbf{x}_{m}$ is denoted by a $q$-dimensional vector $\mathbf{u}_{m} = [u_{m,1}\ u_{m,2}\ \cdots\ u_{m,q}] \in \mathbb{R}^{q}$. Moreover, the state evolution of the plant's non-linear dynamics at time $t = (m+1)\tau_o$ is given as
 \begin{align}
 \label{eq_nonlinear_fn}
 \mathbf{x}_{m+1} &=  \mathbf{f} ( \mathbf{x}_{m},  \mathbf{u}_{m} ) + \mathbf{n}_{s}\\
 &= \mathbf{f}_s( \mathbf{x}_{m} ) + \sum^{q}_{i=1} \mathbf{f}_{u,i} ( \mathbf{x}_{m} ) u_{m,i}  + \mathbf{n}_{s},\label{eq_affine_Control}
 \end{align}
 where $\mathbf{n}_{s} \in \mathbb{R}^{p}$ is a $p$-dimensional random system noise vector at $t = (m+1)\tau_o$. The entries of the noise vector are assumed to be independently and identically distributed (i.i.d.) Gaussian random variables with zero mean and variance $N_{s}$ for all $m\in\mathbb{Z}_{+}$. The function $\mathbf{f}:\mathbb{R}^{p}\times\mathbb{R}^{q} \to \mathbb{R}^{p}$ is a non-linear state transition function of the plant's current state and control action command that steers the plant's state forward in time. Specifically, we introduce a model that disambiguates the state dynamics from the effect of the control actuation by reformulating the non-linear dynamics into a control-affine non-linear system \cite{7799268,korda2018linear}  as \eqref{eq_affine_Control}, where $\mathbf{f}_s(\cdot): \mathbb{R}^{p} \rightarrow \mathbb{R}^{p} $ is the unforced system dynamics and $\mathbf{f}_{u,i}(\cdot): \mathbb{R}^{p} \rightarrow \mathbb{R}^{p}$ is a state dependant control coupling term for $u_{m,i}$ for all $i \in \{1,\dots,q\}$.
 
 
 The time duration between $t = m\tau_o$ and the time point at which an actuator receives the estimated control action command $\hat{\mathbf{u}}_m$ corresponding to the plant's state $\mathbf{x}_m$ is referred to as \emph{control loop duration} and denoted by
 \begin{align}
 \tau_m = \tau_{m,comm} + \tau_{m,comp}
 \end{align}
 for all $m\in\mathbb{Z}_+$. This control loop duration incorporates the communication delay $\tau_{m,comm}$ through forward and reverse links and computing delay $\tau_{m,comp}$ for obtaining the optimal control action command. On the one hand, in the Jacobian baseline, this calls for the forward link to deliver the sampled states to the controller, while the reverse link are also needed for the controller to deliver the obtained control action command to the actuator. On the other hand, in the proposed approach explained in the following section, the system state can be predicted using the trained sensing Koopman AE, thereby only requiring the reverse link as long as the state prediction is accurate.
 
 \subsection{Wireless Communication Model}
 \label{Sensing_and_Actuating_Communications}
Suppose the forward and reverse links follow a time division multiple access (TDMA) approach, and assume that channel reciprocity holds between forward and reverse channels under the assumption that the sensor and actuator are co-located. Moreover, we consider a Rayleigh block fading channel model, where the coherence time is strictly longer than the control loop time. The path-loss of both forward and reverse links is given as
 \begin{align}
     \label{eq_Path_loss}
     \mathrm{PL}_{\mathrm{dB}} \left( D \right)  = \mathrm{PL}_{\mathrm{dB}} \left( D_0 \right)  + 10 \eta\log_{10} \left( \frac{D}{D_0} \right),
 \end{align}
  where $D$ is the distance from sensor and actuator to the controller, $\mathrm{PL}_{\mathrm{dB}} \left( D_o \right)$ denotes the path-loss at the reference distance $D_o$, and $\eta \geq 2$ is the path-loss exponent. Hence the received SNR at the remote controller is given as
 \begin{align}
     \label{eq_SNR_UL}
     \text{SNR}_{m} = 10^{-\frac{\mathrm{PL}_{\mathrm{dB}}\left( D_o \right)}{10}}\frac{P_t | h_{m}|^{2}}{ N_c }\left(\frac{D_o}{D}\right)^{\eta},
 \end{align}
 where $h_{m}$ is the Rayleigh fading channel gain from the sensor to the controller (or the controller to the actuator) at the $m$-th control loop duration, where $|h_{m}|^2$ is exponentially distributed with parameter $\lambda = 1$ for all $m \in \mathbb{Z}_+$, $P_t$ is the transmission power used at both communication ends, and $N_{c}$ is the channel noise power. In addition, we suppose that the channel gains are i.i.d. over time. Having \eqref{eq_SNR_UL}, the transmission rate of both forward and reverse link communications in the control system during the $m$-th control loop can be expressed as
 \begin{align}
     \label{eq_Shannon_data_rate}
     R_{m} = W \log_{2} \left( 1 + \text{SNR}_{m} \right),
 \end{align}
 where $W$ is the communication bandwidth.
 
 To stabilize the control system, the control loop duration should be at least shorter than the control period, that is $\tau_{m} < \tau_{o}$ for all $m \in \mathbb{Z}_{+}$. Denote by $L_{m}$ the overall communicating information bit length in the $m$-th control loop duration, such that $\frac{L_{m}}{R_{m}}$ indicates the communication time. Then, the outage probability of the $m$-th control loop can be expressed as
 \begin{align}
 \epsilon_{m} &= \mathbb{P}\left[ \tau_{m,comm} > \tau_{o} - \tau_{m,comp} \right]\\
 &= 1 - \text{exp} \left[ -10^{\frac{\mathrm{PL}_{\mathrm{dB}}(D_0)}{10}} \frac{ N_c D^{\eta} }{ P_t} \left(2^{ \frac{L_{m}}{W (\tau_{o} - \tau_{m,comp}) } } -1\right)  \right]\label{eq:exp_cumulative}
 \end{align}
 where \eqref{eq:exp_cumulative} holds from the cumulative distribution function (c.d.f.) of the exponential random variable. Note that the control outage probability for each control loop is affected by the communication payload size $L_m$ and computation time $\tau_{m,comp}$ while the other communication parameters in~\eqref{eq:exp_cumulative} are given. Therefore, to reduce the outage probability, the control system should be designed to operate at small communication and computation costs.

==> Closed-Loop Koopman_Camera_Ready/Sec3_Two_Way_Predictive_Control.tex <==
\section{Two-Way Split Koopman Autoencoder Architecture for Predictive Linear Control}
 \label{Split_Closed_Loop_Koopman}
 
 Toward reducing communication and computation costs for closed-loop remote control, we propose a two-way Koopman AE architecture comprised of \emph{sensing and controlling Koopman AEs}. To this end, this section first revisits fundamentals of Koopman operator theory. Then, a split learning method for obtaining a sensing Koopman AE that linearizes the non-linear state dynamics enabling future state prediction at the controller is proposed. Moreover, armed with a well-trained sensing Koopman AE, a linear quadratic regulator (LQR) is applied over the linearized Koopman subspace to obtain the optimal control action command at a small computational cost. In addition, we propose a split learning-based controlling Koopman AE that predicts future control action commands at the actuator.
 
\subsection{Preliminary: Koopman Operator for Closed-Loop Control}
\label{Basics_Theory_of_Closed-loop_Koopman_operator}

 Typically, a data sample observed from a closed-loop controlled dynamical system can be seen as a function of a system state and control action. Define functions $g:\mathbb{R}^{p}\times\mathbb{R}^{q}\rightarrow \mathbb{R}$, dubbed \emph{observables} which span an infinite-dimensional Hilbert space $\mathcal{H}$. The Koopman operator $\mathcal{K}:\mathcal{H}\to\mathcal{H}$ is a linear operator that acts on $\mathcal{H}$ \cite{proctor2018generalizing,brunton2021modern} such that
\begin{align}
     \label{eq_Koopman_Composition}
     \mathcal{K} g ( \mathbf{x}_{m}, \mathbf{u}_{m} ) = g ( \mathbf{f}( \mathbf{x}_{m}, \mathbf{u}_{m} ),  \mathbf{u}_{m+1} ),
 \end{align}
 for some observable $g$. Note that by ignoring the additive system noise in \eqref{eq_nonlinear_fn}, the expression \eqref{eq_Koopman_Composition} can be rewritten as 
 \begin{align}\label{eq:noiselessKoopman}
 \mathcal{K}  g ( \mathbf{x}_{m}, \mathbf{u}_{m} ) = g ( \mathbf{x}_{m+1}, \mathbf{u}_{m+1}),
 \end{align}
 and in other words, the Koopman operator in \eqref{eq:noiselessKoopman} enables to express the linear evolution of the non-linear system dynamics in the function space $\mathcal{G}$. However, to obtain the Koopman operator, representation and computation issues may raise, since the operator acts on the infinite dimensional space $\mathcal{H}$.
 
 One approach to resolve such problems is to find an invariant subspace spanned by a finite set of functions. That is, finding a span of $d$ different functions $\{g_1,g_2, \dots g_d\}$, such that a function $g$ in this subspace
 \begin{align}
 \label{eq_Eigenfunctions_Span}
 g(\mathbf{x}_{m}, \mathbf{u}_{m}) = a_1g_1(\mathbf{x}_{m}, \mathbf{u}_{m}) +  \cdots + a_d g_d(\mathbf{x}_{m}, \mathbf{u}_{m}),
 \end{align}
 for some real-valued coefficients $a_1,\dots,a_d \in \mathbb{R}$, is still in the same subspace after acted on by the Koopman operation
 \begin{align}
 \label{eq_Koopman_Eigs}
 \mathcal{K}g(\mathbf{x}_{m}, \mathbf{u}_{m}) = b_1 g_1(\mathbf{x}_{m},\mathbf{u}_{m}) + \cdots+ b_d g_d(\mathbf{x}_{m}, \mathbf{u}_{m}),
 \end{align}
 for some real-valued coefficients $b_1,\dots,b_d \in \mathbb{R}$. Note that the Koopman operator is linear and thus allows eigendecomposition, and any finite set of eigenfunctions of the Koopman operator will span an Koopman invariant subspace \cite{kaiser2017data}. Therefore, by introducing a finite-dimensional Koopman matrix representation $\mathbf{K} \in \mathbb{R}^{d \times d}$ for a given Koopman invariant subspace, we can obtain a global linearization expression of a non-linear system dynamics in~\eqref{eq_nonlinear_fn} as 
 \begin{align}
     \label{eq_Koopman_Linear}
     \mathbf{g}(\mathbf{x}_{m+1}, \mathbf{u}_{m+1}) = \mathbf{K} \mathbf{g}(\mathbf{x}_{m}, \mathbf{u}_{m}),
 \end{align}
 where $\mathbf{g}$ is the $d$-dimensional vector of which the elements are the Koopman eigenfunctions. Note that for a given current system state $\mathbf{x}_{m}$ and its computed control action command $\mathbf{u}_{m}$, if the concatenated eigenfunctions $\mathbf{g}$, its element-wise inverse $\mathbf{g}^{-1}$, and the Koopman matrix $\mathbf{K}$ are known, the future system state $\mathbf{x}_{m+1}$ and control action command $\mathbf{u}_{m+1}$ can be readily obtained. However, since discovering the Koopman eigenfunctions from finite samples of a dynamical system is still challenging, it calls for an autoencoder-based deep learning based approach as will be explained in the following subsections.
 
 In the meantime, since the control system exhibits control-affine non-linear dynamics in \eqref{eq_affine_Control} in this article, the global linearization expression \eqref{eq_Koopman_Linear} can be recast as~\cite{kaiser2017data}
 \begin{align}
     \label{eq_Koopman_non_Affine}
     \begin{bmatrix}
     \mathbf{g}_s( \mathbf{x}_{m+1} ) \\ 
     \mathbf{g}_u( \mathbf{x}_{m+1},\mathbf{u}_{m+1} )
     \end{bmatrix} =  \mathbf{K}  \begin{bmatrix}
     \mathbf{g}_s ( \mathbf{x}_{m} ) \\ 
     \mathbf{g}_u ( \mathbf{x}_{m},\mathbf{u}_{m})
     \end{bmatrix},
 \end{align}
 where $\mathbf{g}_s$ is the $d$-dimensional vector of Koopman eigenfunctions that depend only on the system states, $\mathbf{g}_u$ is the $f$-dimensional vector of Koopman eigenfunctions that depend on both system states and control action commands. For the purpose of utilizing linear control theory, it is required to ensure that the linear evolution of the Koopman eigenfunctions is explicitly related to the control action commands; hence we simplify $\mathbf{g}_u$ in~\eqref{eq_Koopman_non_Affine} into $\mathbf{g}_u ( \mathbf{x}_{m},\mathbf{u}_{m}) \approx \mathbf{u}_{m}$, and thus \eqref{eq_Koopman_non_Affine} becomes \cite{mamakoukas2019local,bonnert2020estimating, kaiser2017data}
 \begin{align}
     \label{eq_Koopman_Simplification}
     \begin{bmatrix}
     \mathbf{g}_s(\mathbf{x}_{m+1})\\ \mathbf{u}_{m+1}
     \end{bmatrix}
     = \begin{bmatrix}
      \mathbf{K}_{11}  \; \;  \mathbf{K}_{12} \\
      \mathbf{K}_{21}  \; \;  \mathbf{K}_{22}
     \end{bmatrix} \begin{bmatrix}
     \mathbf{g}_s(\mathbf{x}_{m})\\ \mathbf{u}_{m}
     \end{bmatrix},
 \end{align} where $\mathbf{g}_s$ and $\mathbf{g}$ are used interchangeably thereafter, $\mathbf{K}_{11} \in \mathbb{R}^{d \times d}$ is the state transition matrix in the Koopman matrix $\mathbf{K} \in \mathbb{R}^{d+q}\times\mathbb{R}^{d+q}$, $\mathbf{K}_{12} \in \mathbb{R}^{d \times q}$ is the control action matrix of the state dynamics, $\mathbf{K}_{21} \in \mathbb{R}^{q \times d}$ is the state-dependent control action matrix, and $\mathbf{K}_{22} \in \mathbb{R}^{q \times q}$ is the control action matrix of the control dynamics. Moreover, we define $\mathbf{K}_{s} = \left[ \mathbf{K}_{11} \; \mathbf{K}_{12} \right]$ as the state Koopman matrix representing the state dynamics, while $\mathbf{K}_{a} = \left[ \mathbf{K}_{21} \;  \mathbf{K}_{22} \right]$ as the action Koopman matrix representing the control action dynamics. Note that the simplification of~\eqref{eq_Koopman_non_Affine} in~\eqref{eq_Koopman_Simplification} comes at the cost of less accurate approximation of the system dynamics. For instance, if the term $\sin(x_{m,1}) \mathbf{u}_{m}$ appears in the system dynamics, it will be approximated in the Koopman model as $c_{1}\mathbf{u}_{m}$, where $c_{1} \in \mathbb{R}$ is a constant.

 \subsection{Sensing Koopman Autoencoder for State Prediction}
 \label{Wireless_Split_Closed-loop_Koopman_Auto-encoder}
 The first component of the two-way Koopman AE architecture is the \emph{sensing Koopman AE}, which plays two roles: (i) linearizing the non-linear system dynamics and (ii) predicting the future system states based on the linearized system dynamics.
 Note that linearization of non-linear system dynamics helps reduce the complexity in terms of minimizing the computational time required to analyze the system and calculate its optimal control action command, while state prediction helps reduce the communication cost~\cite{guastello2009introduction}. The proposed sensing Koopman AE is a tripartite neural network that consists of an \textit{encoder} that is related to the concatenated Koopman eigenfunctions
 $\mathbf{g}$, two fully-connected hidden layers that constitute a finite-dimensional matrix representation of the Koopman operator $\mathbf{K}$, and the \textit{decoder} which is an inverse function vector of the encoder $\mathbf{g}^{-1}$. Since we consider a remote control scenario, the Koopman AE is split into two parts, where the encoder is located at the sensor and actuator side, while the Koopman hidden layers and the decoder are situated at the controller side. Thus, the sensing Koopman AE is trained through split learning~\cite{Vepakomma:2018:Splita,koda2020communication} which will be detailed in Section \ref{Split_Closed-loop_Koopman_Training}.
 
 Once the sensing Koopman AE is trained, the sensor sends an encoded representation $\mathbf{g}(\mathbf{x}_{m})$ of the sampled system state $\mathbf{x}_{m}$ and the controller obtains an estimated latent state representation $\hat{\mathbf{g}}(\mathbf{x}_{m})$ and concatenates it with the computed control action command $\mathbf{u}_{m}$ as $\mathbf{y}_{m} = [ \hat{\mathbf{g}}(\mathbf{x}_{m})\  \mathbf{u}_{m}]^{\mathsf{T}} $. Then, by multiplying $\mathbf{y}_{m}$ with the sensing Koopman operator matrix $\mathbf{K}_{s}$, the remote controller obtains a linear state representation evolution as \begin{align}
   \label{eq_linear_evol_Representation}
      \hat{\mathbf{g}}(\mathbf{x}_{m+1})  = \mathbf{K}_{11} \hat{\mathbf{g}}(\mathbf{x}_{m}) + \mathbf{K}_{12} \mathbf{u}_{m}, 
   \end{align}
   where $\mathbf{K}_{11}$ and $\mathbf{K}_{12}$ are the Koopman submatrices mentioned in \eqref{eq_Koopman_Simplification}. Moreover, by passing $\mathbf{y}_{m}$ through the trained sensing Koopman matrix and the decoder, the remote controller obtains the predicted future system state as $\bar{\mathbf{x}}_{m+1} = \mathbf{g}^{-1}(\mathbf{K}_{s} \mathbf{y}_{m})$. Moreover, by multiplying the sensing Koopman matrix $m'$ times, the controller can predict the future system states at $t = (m+m')\tau_o$ as
   \begin{align}
       \label{eq_predicted_states}
       \bar{\mathbf{x}}_{m + m'} = \mathbf{g}^{-1} (\mathbf{K}_{s}^{m'} \mathbf{y}_{m}),
   \end{align} for all target prediction depth $m' \in \mathbb{Z}_+$ which will be detailed in Section~\ref{Koopman-based_Controller}. 
   
   To this end, the proposed real-time remote control of a closed-loop control system, aided by the Koopman AE, consists of two-phases. In the first phase, the remote controller receives the measured system states in real-time from the sensor, computes its control action command, and sends it back to the actuator. Meanwhile, the sensor and controller train the sensing Koopman AE and the first phase is maintained until it is well-trained. In the second phase, the remote controller sends back a control signal informing the sensor to stop sending the system states once it is well-trained, and since the sensing Koopman AE is trained, the remote controller can predict the future system states.
   
   
 \subsection{Linear Control over Koopman Subspace}
 \label{Koopman-based_Controller}
 
  Having a closed-loop Koopman AE, an optimal control action can be computed over the linearized Koopman subspace by readily applying linear control theory. That is, formulating an infinite-horizon discrete-time linear quadratic regulator (LQR) over the linearized Koopman subspace rather than over the non-linear system dynamics. Following~\cite{brunton2016koopman}, the control objective is a quadratic cost function given as \begin{align}
       \label{eq_lqr_objective}
        \mathcal{J}(\hat{\mathbf{g}} (\mathbf{x}_{m}),\mathbf{u}_{m}) = \frac{1}{2} \sum^{\infty}_{m=0} \hat{\mathbf{g}}(\mathbf{x}_{m})^{\mathsf{T}} \mathbf{Q}_{g} \hat{\mathbf{g}}(\mathbf{x}_{m})  + \mathbf{u}^{ \mathsf{T}}_{m} \mathbf{R} \mathbf{u}_{m},
  \end{align}
  where $\mathbf{Q}_{g} \in \mathbb{S}_{+}^{d \times d}$ is a positive semi-definite weight matrix of the latent state representation deviation cost, and $\mathbf{R} \in \mathbb{S}_{++}^{q \times q}$ is a positive definite weight matrix of the control action cost. Then, the optimization problem of an infinite-horizon discrete-time LQR to calculate the optimal control action is formulated as \vspace{-8pt} \begin{subequations} \label{eq_LQR_Optimization_1} \begin{gather} \label{eq_LQR_Optimization}
  \underset{\hspace{-95pt}\mathbf{u}_{m}}{ \hspace{-100pt} \text{Minimize}} \hspace{-10pt} \mathcal{J}(\hat{\mathbf{g}}(\mathbf{x}_{m}),\mathbf{u}_{m}) \\
  \hspace{15pt} \text{subject to:}\; \;   \hat{\mathbf{g}}(\mathbf{x}_{m+1}) = \mathbf{K}_{11} \hat{\mathbf{g}}(\mathbf{x}_{m}) + \mathbf{K}_{12} \mathbf{u}_{m}. \label{eq_LQR_Optimization_a}  
  \end{gather}\end{subequations} 
  The problem in~\eqref{eq_LQR_Optimization_1} is a convex optimization problem with a quadratic cost function and linear constraint, hence the optimal control action can be readily obtained as
  \begin{align}
     \label{eq_optimal_control_law}
     \mathbf{u}_{m} = - \mathbf{K}_{\mathrm{LQR}} \; \hat{\mathbf{g}}(\mathbf{x}_{m}), 
  \end{align} 
  where $\mathbf{K}_{\mathrm{LQR}} \hspace{-20pt} = \hspace{-20pt} \left( \mathbf{R} + \mathbf{K}_{12}^{\mathsf{T}} \mathbf{P} \mathbf{K}_{12} \right)^{-1}  \mathbf{K}_{12}^{\mathsf{T}}  \mathbf{P} \mathbf{K}_{11}^{\mathsf{T}} $ is the feedback gain matrix, and $\mathbf{P} \hspace{-15pt} = \hspace{-15pt} \mathbf{K}_{11}^{\mathsf{T}}  \mathbf{P} \mathbf{K}_{11}  - \mathbf{K}_{11}^{\mathsf{T}}  \mathbf{P} \mathbf{K}_{12}  \left( \mathbf{K}_{12}^{\mathsf{T}}  \mathbf{P} \mathbf{K}_{12}  + \mathbf{R} \right)^{-1} \mathbf{K}_{12}^{\mathsf{T}}  \mathbf{P} \mathbf{K}_{11}  + \mathbf{Q}_{g}$ is a unique positive definite matrix which satisfies the discrete-time algebraic Riccati equation (DARE)~\cite{bemporad2002explicit}. The Koopman-based controller outperforms the locally linearized-based controller in terms of control performance. This is because the locally linearized-based controller performs optimally near the equilibrium point, but the performance becomes poor for the points that are located far from the equilibrium point. In contrast, since the Koopman operator globally linearizes the system dynamics, the controller over the linearized Koopman subspace performs optimally for all points.

  \subsection{Split Learning-based Koopman Autoencoder}
  \label{Split_Closed-loop_Koopman_Training}
  
  An optimization problem for obtaining the closed-loop Koopman AE in the considered WNCS can be formulated as
  \begin{subequations}  \label{eq_training_Optimization_ab} \begin{gather} \label{eq_training_Optimization}
  \underset{\mathbf{K}, \mathbf{g},\mathbf{g}^{-1} }{ \textrm{minimize}} \;  \frac{1}{M_{d}} \sum_{m' = 1}^{M_d} \left\lVert \hat{\mathbf{x}}_{m+m'} - \sum_{l = 0}^{M_d - 1} \mathbf{g}^{-1} \left( \mathbf{K}_{s}^{ M_{d} - l } \mathbf{y}_{m + l} \right) w_{l} \right\rVert_{2}^{2} \\
  \hspace{-130pt} \text{subject to:}\; \;   \bar{\mathbf{x}}_{m} = \mathbf{g}^{-1} \left( \mathbf{y}_{m} \right) , \label{eq_training_Optimization_a}  
  \end{gather}\end{subequations} where $\hat{\mathbf{x}}_{m+m'}$ is the estimated system state at time $m+m'$, $M_d$ is the target prediction depth considered in the training that represents the Koopman operator prediction time horizon checked in the training, and $w_{l}$ is a weight parameter of the $l$-th predicted system state at the controller side. On the one hand, when $l = 0 $ and $w_{l} = 1$, we call it a \textit{special case} of the optimization problem in~\eqref{eq_training_Optimization_ab} suggested in~\cite{lusch2018deep,xiao2020deep}. On the other hand, when $l > 0$ and $w_{l} = 1 / M_{d}$, we call it a \textit{general case} of the optimization problem in~\eqref{eq_training_Optimization_ab} proposed in this paper. The \textit{general case} of the optimization problem in~\eqref{eq_training_Optimization_ab} utilizes all the received latent state representations to predict the future system states compared to the \textit{special case}. Since it is analytically hard to solve the formulated optimization problem in~\eqref{eq_training_Optimization_ab} for long-term target prediction depth, we solve it by exploiting deep learning over three separated unconstrained optimization sub-problems formulated as follow. 

  %\tred{[Is this your proposition or did you get if from the other paper? If you got it from the others this statement makes plagiarism issue.]} The loss functions of these separated optimization sub-problems are formulated as follows. \tred{[Why do you enumerate three losses while you have four?]}
  \begin{enumerate}
        \item A \textit{reconstruction loss} is formulated to accurately reconstruct the system states. This loss measures the mean squared error (MSE) between the estimated system states $\hat{\mathbf{x}}_{m}$ and the decoded estimated state representation adjoined with the control action command $\mathbf{g}^{-1}(\mathbf{y}_{m})$, given as 
        \begin{align}
            \label{eq_Reconst_loss}
            \mathcal{L}_{1} = \frac{1}{M_s} \sum_{m = 1}^{M_{s}} || \hat{\mathbf{x}}_{m} - \mathbf{g}^{-1} \left(\mathbf{y}_{m} \right) ||^{2}_2, 
        \end{align} where $M_{s}$ denotes the length of the received time-series signals in the first phase of the remote control of a closed-loop control system.
        
        \item A \textit{linear Dynamics loss} is formulated to obtain the linear finite-dimensional sensing Koopman matrix $\mathbf{K}_{s}$ that ensures the linearity in the Koopman invariant subspace. This loss measures the MSE between the estimated state representation of the future system state adjoined with its future control action commands as $\mathbf{y}_{m + m'}$ and the weighted sum of the multiplication of the sensing Koopman matrix with different target prediction depth during training and the estimated state representation of the received system states adjoined with the calculated control action commands $ \sum_{l = 0}^{M_d - 1} \left( \mathbf{K}_{s}^{ M_{d} - l } \mathbf{y}_{m + l} \right) w_{l} $, i.e., \begin{align}
            \label{eq_Linear_Loss}
            \mathcal{L}_{2} = \frac{1}{M_{d}} \sum_{m' = 1}^{M_d} ||  \mathbf{y}_{m+m'} - \sum_{ l = 0}^{M_d - 1} \left( \mathbf{K}_{s}^{ M_{d} - l} \mathbf{y}_{m + l} \right) w_{l} ||_{2}^{2}.
        \end{align} Note that the linear latent state representation evolution in~\eqref{eq_Linear_Loss} for $l = 0$ is represented as  $\mathbf{K}_{s}^{M_{d}} \mathbf{y}_{m} = \mathbf{K}_{11}^{M_{d}} \mathbf{g}(\mathbf{x}_{m}) + \sum^{M_{d}}_{m'=1} \mathbf{K}_{11}^{m'-1} \mathbf{K}_{12} \mathbf{u}_{m+m'-1}$. 
        
    
        \item A \emph{prediction loss} is formulated to accurately predict the future system states. The prediction loss measures the MSE between the estimated future system states $\hat{\mathbf{x}}_{m+m'}$ and decoded weighted sum of the multiplication of the sensing Koopman matrix with different target prediction depth considered in training and the estimated state representation of the received system states adjoined with the calculated control action commands $ \mathbf{g}^{-1}(\sum_{ l = 0}^{M_d - 1} \left( \mathbf{K}_{s}^{ M_{d} - l } \mathbf{y}_{m + l} \right) w_{l})$, i.e., 
         \begin{align}
            \label{eq_Pred_loss}
            \mathcal{L}_{3} = \frac{1}{M_{d}} \sum_{m' = 1}^{M_d} || \hat{ \mathbf{x}}_{m+m'} - \bar{\mathbf{x}}_{m + m'}  ||_{2}^{2},
         \end{align}
        where the future predicted system state $ \bar{\mathbf{x}}_{m + m'}$ in~\eqref{eq_Pred_loss} is given as  $ \bar{\mathbf{x}}_{m + m'} = \sum_{ l = 0}^{M_d - 1}  \mathbf{g}^{-1} \left( \mathbf{K}_{s}^{ M_{d} - l } \mathbf{y}_{m + l} \right)  w_{l}$.
        
        
        \item A \textit{representation cost loss} is formulated to guarantee that the state representation deviation cost is equivalent to the system state deviation cost in the Jacobian linearization method. This loss measures the MSE between the state representation deviation cost $\tilde{\mathbf{Q}}_{g}$ and the system state deviation cost $\mathbf{Q}_{x}$, given as
  \begin{align}
            \label{eq_representation_cost}
            \mathcal{L}_{4} = \frac{1}{M_{s}} \sum_{m = 1}^{M_{s}} || \hat{ \mathbf{x}}_{m}  \mathbf{Q}_{x}  \hat{\mathbf{x}}_{m} -  \hat{ \mathbf{g}}(\mathbf{x}_{m}) \tilde{\mathbf{Q}}_{g} \hat{\mathbf{g}}(\mathbf{x}_{m}) ||_{2}^{2}.
    \end{align} Here, we set $\mathbf{Q}_{g} = [\tilde{\mathbf{Q}}_{g}]_{+}$ as the final estimator, where $[.]_{+}$ truncates the non-positive eigenvalues to zero to ensure the state representation deviation cost is a positive semi-definite weight matrix.
    \end{enumerate} 
    
 Overall, the total weighted-sum loss function to train the closed-loop Koopman AE for predicting the future system states and calculating the optimal control action is given as 
    \begin{align}
       \label{eq_Updated_Overall_loss}
       \mathcal{L} = c_{1} \mathcal{L}_{1} + c_{2} \mathcal{L}_{2} + c_{3} \mathcal{L}_{3} +  c_{4} \mathcal{L}_{4},
    \end{align}
    for some positive coefficients $c_{1}, c_{2}, c_{3}, c_4 \in \mathbb{Z}_+$. The weights of the sensing Koopman AE can be trained based on the stochastic gradient descent (SGD) and backpropagation via feedback channels from the controller to the sensor. An early stopping strategy is utilized to avoid model overfitting, which enhances both the prediction accuracy and communication efficiency. Note that the sensor must consistently sample the system states and send them along with the latent state representations to the controller over wireless fading channels during the first phase of remote control to compute the total weighted-sum loss at the remote controller. Otherwise, if the system states are missed due to adverse channel conditions in the forward link, the remote controller predicts the future system states based on the last observed system states.
    
 \subsection{Controlling Koopman Autoencoder for Control Prediction}
 \label{Wireless_Split_Input_Closed-loop Koopman_Auto-encoder}
 
  To compensate for the missing control action command in case of adverse channel conditions in the reverse link, we propose controlling Koopman AE to linearize the action dynamics and predict the future control action commands at the actuator side. The proposed controlling Koopman AE is composed of three parts of the encoder that is located at the sensor side is the same as the encoder utilized in the sensing Koopman AE $\mathbf{g}$, the Koopman hidden layers at the actuator side $\mathbf{K}'$, and the decoder are located at the actuator side $\mathbf{g}_{a}^{-1}$. After the controlling Koopman AE is well-trained, if the remote controller sends a control action command $\mathbf{u}_{m}$, the actuator obtains a noisy control action command $\hat{\mathbf{u}}_{m}$, applies it on the plant, and concatenates it with the latent state representations $\mathbf{g}(\mathbf{x}_{m})$ as follows $\mathbf{z}_{m} = [ \mathbf{g}(\mathbf{x}_{m}) \; \;  \hat{\mathbf{u}}_{m}]^{\mathsf{T}} $. Then, by passing $\mathbf{z}_{m}$ through the finite-dimensional controlling Koopman matrix $\mathbf{K}'_{a}$, the linear control action command evolution at the actuator is given as
  \begin{align}
   \label{eq_linear_evol_input}
    \hat{\mathbf{u}}_{m+1} =
    \mathbf{K}'_{21} \mathbf{g}(\mathbf{x}_{m}) + \mathbf{K}'_{22} \hat{\mathbf{u}}_{m},  
   \end{align} where $\mathbf{K}'_{21} \in \mathbb{R}^{q \times d}$ and $\mathbf{K}'_{22} \in \mathbb{R}^{q \times q}$ are the trained Koopman submatrices at the actuator side representing the non-linear control action dynamics. 
   
   Since the objective of the controlling Koopman AE is to predict the future control action commands for a long time, it is required to have the measurement functions, its inverse functions, and the finite-dimensional Koopman matrix. Therefore, we train the controlling Koopman AE through an optimization problem formulated as 
   \begin{subequations}  \label{eq_actuating_Optimization_ab} \begin{gather} \label{eq_actuating_Optimization}
  \underset{\mathbf{K}', \mathbf{g},\mathbf{g}_{a}^{-1} }{ \text{minimize}} \hspace{8pt}  \frac{1}{M_{d}}  \sum_{m' = 1}^{M_d} ||\mathbf{x}_{m+m'} - \tilde{\mathbf{x}}_{m + m'} ||_{2}^{2} \\
  \hspace{-80pt} \text{subject to:}\; \;   \tilde{\mathbf{x}}_{m} = \mathbf{g}_{a}^{-1} \left( \mathbf{z}_{m} \right) , \label{eq_actuating_Optimization_a}  
  \end{gather}\end{subequations}  where  $\tilde{\mathbf{x}}_{m + m'} = \sum_{l = 0}^{M_d - 1} \mathbf{g}_{a}^{-1} \left( \mathbf{K}_{a}'^{{M_{d} - l} } \mathbf{z}_{m + l} \right) w'_{l}$ is the future predicted system states at the actuator side, and $w'_{l}$ is the $l$-th weight parameter of the predicted system state at the actuator. The problem in~\eqref{eq_actuating_Optimization_ab} is similar to the problem of the sensing Koopman AE in~\eqref{eq_training_Optimization_ab} except that the controlling Koopman AE receive noisy control action commands and the original system states along with their state representations. As a result, we minimize a total weighted-sum of three separated loss functions similar to the sensing Koopman AE given as  \begin{align}
       \label{eq_Overall_input_loss}
       \mathcal{L}' = c_{1}' \mathcal{L}'_{1} + c_{2}' \mathcal{L}'_{2} + c_{3}' \mathcal{L}'_{3},
   \end{align} where $c_{1}'$, $c_{2}'$, and $c_{3}'$ are positive weighting hyperparameters of the controlling Koopman AE. The loss functions $\mathcal{L}_{1}'$, $\mathcal{L}_{2}'$, and $\mathcal{L}_{3}'$ of the controlling Koopman AE in~\eqref{eq_Overall_input_loss} are similar to the loss functions $\mathcal{L}_{1}$, $\mathcal{L}_{2}$, and $\mathcal{L}_{3}$ of the sensing Koopman AE,  respectively except that $\hat{\mathbf{x}}_{m}$ is substituted by $\mathbf{x}_{m}$ and $\mathbf{y}_{m}$ by $\mathbf{z}_{m}$.
   
 %\begin{algorithm}  
 %\caption{Split closed-loop Koopman Autoencoder}\label{alg:euclid}
% {\small\begin{algorithmic}[1]
% \State initialize $\mathbf{K}_{s}$, $\mathbf{K}'_{a}$, and $x,v,\theta,\omega \in [-0.5,0.5]$;
% \For{\textbf{all} epochs}
%  \For{\textbf{all} batches }
 %\State observe the wireless channels $ H^{ij}_{m}$ ;
% \State obtain $\hat{\mathbf{x}}_{m}$ and compute $\mathbf{u}_{m} $;
% \State obtain $\hat{\mathbf{u}}_{m}$ and apply it on~\eqref{eq_nonlinear_fn};
% \State minimize $\mathcal{L}$ and $\mathcal{L}' $;
% \State update $\mathbf{K}_{s}$, $\mathbf{K}'_{a}$ via  backpropagation;
% \EndFor
% \EndFor
% \State obtain $\mathbf{K}_{11}$ and $\mathbf{K}_{12}$;
% \State predict $\bar{\mathbf{x}}_{m +m'}$, $\forall m' \geq m$;
% \State obtain $\mathbf{Q}_{g}$ and choose $\mathbf{R}$;
% \State calculate $\mathbf{u}_{m}$ and apply it on~\eqref{eq_nonlinear_fn};
% \State obtain $\mathbf{K}'_{21}$ and $\mathbf{K}'_{22}$;
% \State predict $\bar{\mathbf{u}}_{m +m'}$, $\forall m' \geq m$;
% \end{algorithmic}\normalsize }
% \end{algorithm}  

==> Closed-Loop Koopman_Camera_Ready/Sec4_Simulation_Results.tex <==
 \section{Simulation Results and Discussion}
 \label{Simulation_Results}

  In this section, we investigate the performance of both sensing Koopman AE and controlling Koopman AE over wireless fading channels in an inverted cart-pole system. This control system is non-linear and multi-dimensional. For a given time, the inverted cart-pole system is described by a four-dimensional state vector $\mathbf{x} = [ x \; v \;  \theta \; \omega ]^{T}$, where $x$ and $v$ represent the horizontal position and velocity of the cart, respectively. The terms $\theta$ and $\omega$ are the vertical angle and angular velocity of the pendulum, respectively. The control action is described as a horizontal force applied on the cart $u$. Accordingly, the full non-linear system dynamics is described as follows.    
  \begin{align}\label{CIP_Dynamics}
  \begin{split}
  \frac{dx}{dt} &= v,\\
  \frac{d \theta}{dt}  &= \omega, \\
  \frac{dv}{dt} &= \frac{-m_{p}^{2} L^{2} \nu \; c\theta \; s\theta + m_{p} L^{2} (m_{p} L\omega^{2} s\theta - \delta v )  + m_{p} L^{2} u }{m_{p} L^{2} \left(m_{c} + m_{p} (1 - c\theta^{2} ) \right)},\\
  \frac{d \omega}{dt} & = \frac{ m_{pm} m_{p} \nu L s\theta - m_{p} L c\theta ( m_{p} L\omega^{2} s\theta - \delta v ) + m_{p} L c\theta u}{ m_{p} L^{2} \left( m_{c} + m_{p} ( 1 - c\theta^{2} )\right)},
 \end{split}
 \end{align} with $m_{pm} = m_{p} + m_{m}$, $c\theta = \cos(\theta)$,  and $s\theta = \sin(\theta)$. Here, we consider the following simulation parameters unless stated otherwise: pendulum mass $m_{p} = 1$ $\mathrm{Kg}$, cart mass $m_{c} = 5$ $\mathrm{Kg}$, pendulum length $L = 0.2$ $\mathrm{m}$, gravitational acceleration $\nu = -10$  $\mathrm{m/} \mathrm{s}^{2}$, and cart damping $\delta = -2$ $\mathrm{N s} /\mathrm{m}$. 
 
 \subsection{Data Generation and Training}
 \label{Dataset}
 
 The training dataset of the sensing Koopman AE is generated at the controller based on the calculated control action commands and the received system states from the inverted-cart pole system with a sampling rate of $\tau_{0} =  10$ $\mathrm{ms}$ in the time interval $m \in [0, |\mathcal{M}_{\mathrm{Train}}|]$ and with a random initial condition in the range of $[-0.5,0.5]$ for each state dimension. For each initial condition, we solve the system of differential equations in~\eqref{CIP_Dynamics} using the fourth-order Runge Kutta numerical method with $0.01$ equally-spaced step size and trajectory length of $\mathcal{M}_{\mathrm{Train}} = 250$ $\mathrm{s}$. The training dataset consists of $T_{t} = 70$, the validation dataset of $T_{v} = 20$, and the test dataset of $T_{e} = 10$ trajectories. The AE weights are initialized with a normal distribution of the form $w \sim \mathcal{N} ( 0, \frac{2}{d_{in}} )$ where $d_{in}$ is the number of neurons of the input layer. The autoencoder weights are trained to minimize the total weighted sum loss in~\eqref{eq_Updated_Overall_loss} for the sensing Koopman AE, via Adam optimizer~\cite{sutskever2013importance} with batch size of $64$ and learning rate of $10^{-4}$. The encoder of the sensing Koopman AE consists of three fully-connected layers that contain $128, 64, 32$ neurons with rectified linear unit (ReLu) activation, respectively, and the final layer contains $d$ neurons with linear activation. The decoder begins with $2$ fully-connected layers with the width $(d+q) \in \{2, 3, 4, 5\}$ (i.e., latent state representation dimension plus control action command dimension) and the rest follows the same structure of the encoder. The weighting hyperparameters of the sensing Koopman AE are set as $c_{1} = c_{3} = 0.5,$ $c_{2} = c_{4} = 1$. The wireless communication channels are assumed to follow Rayleigh fading channels. Here, the results are obtained based on the model with the lowest validation error of several training runs. We consider a maximum transmission power value of $P_{t} = 20$ $\mathrm{dBm}$, different SNR of $\mathrm{SNR} \in \{-10, 0, 10, 20\}$ $\mathrm{dBm}$, distance between transmitter-receiver pair of $D = 100 \, \mathrm{m}$, and the path-loss exponent of $\eta = 3$. The dataset of the controlling Koopman AE is generated at the actuator based on the system states and the received control action commands from the controller. The rest follows the same structure of the sensing Koopman AE with hyperparameters set as 

  \begin{figure*}[t]
    \centering
    \subfigure[Cart Position.]{\includegraphics[width=0.4\textwidth]{Fig/Cart_Poisition_Vs_SNR.eps}} 
    \subfigure[Cart Velocity.]{\includegraphics[width=0.4\textwidth]{Fig/Cart_Velocity_Vs_SNR.eps}} 
   \subfigure[Pendulum Angular Position.]{\includegraphics[width=0.4\textwidth]{Fig/Pendulum_Angle_Vs_SNR_1.eps}}
    \subfigure[Pendulum Angular Velocity.]{\includegraphics[width=0.4\textwidth]{Fig/Pendulum_Velocity_Vs_SNR_1.eps}}
   \caption{Time-series of the predicted inverted cart-pole system states utilizing the proposed sensing Koopman autoencoder before observing the ground truth.}
    \label{fig state_prediction}
\end{figure*} 
 
  \begin{figure}[t]
   \centering
   \includegraphics[ width=0.4\textwidth]{Fig/Applied_Force_3.eps} \\
   \caption{Time-series of predicted force applied on the cart utilizing the proposed controlling Koopman autoencoder before observing the ground truth.} \label{fig_force}
  \end{figure}
 
 \subsection{Evaluation Metrics}
 \label{Evaluaion Metric}
  In this subsection, we present the evaluation metrics used to evaluate the proposed sensing Koopman AE and the controlling Koopman AE according to different evaluation metrics in terms of prediction accuracy, wireless communication efficiency, and control stability.


 \begin{table*}[t]
    \centering
   \caption{ State and Action Prediction NRMSE for different latent state representation dimensions and SNR.}
    \label{Table_1}
\begin{tabularx}{1\linewidth}{p{1.5cm} p{2cm} p{2cm} p{4cm} p{4cm}}
    \toprule[1pt]
    & Representation Dimensions $d$   & SNR [dBm]  & State Prediction NRMSE [\%] & Action Prediction NRMSE [\%] \\     
    \cmidrule(r){2-2} \cmidrule(r){3-3} \cmidrule(r){4-4} \cmidrule(r){5-5}
  & \qquad $1$   &  $ \quad -10$   & $14.38$ \hspace{5pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (2.7,0.2);
    } &  $8.97$ \hspace{9pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (1.56,0.2);
        }\\
  &   & $\qquad \; 0$  & $ 14.15$ \hspace{5pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (2.65,0.2);
    } & $3.87$ \hspace{9pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.78,0.2);
    } \\
   &   & $\qquad 10$ & $13.89$ \hspace{5pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (2.60,0.2);
     } & $0.99$ \hspace{9pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.27,0.2);
     } \\
 &    &  $\qquad  20$  & $\mathbf{9.20}$ \hspace{7pt}  \tikz{
        \fill[fill=color4] (0.0,0) rectangle (2.1,0.2);
    }   & $\mathbf{0.55}$ \hspace{7.5pt}  \tikz{
        \fill[fill=color9] (0.0,0) rectangle (0.21,0.2);
    } \\ \hline
 & \qquad  $2$ &  $ \quad-10$  & $6.69$\; \hspace{7pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (1.16,0.2);
    }  & $9.08$\; \hspace{7pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (1.61,0.2);
    } \\
  &    &  $\qquad \; 0$  & $5.79$\; \hspace{7pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (1.06,0.2);
    } & $3.85$\; \hspace{7pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.8,0.2);
    }  \\ 
   &  &  $\qquad 10$  & $5.18$\; \hspace{7pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (0.98,0.2);
    } & $0.99$\; \hspace{7pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.27,0.2);
    } \\ 
 &    &  $\qquad 20$  & $\mathbf{4.93}$ \hspace{7pt}  \tikz{
        \fill[fill=color4] (0.0,0) rectangle (0.95,0.2);
    }  & $\mathbf{0.52}$ \hspace{7pt}  \tikz{
        \fill[fill=color9] (0.0,0) rectangle (0.19,0.2);
    }  \\ \hline
   & \qquad $3$ &  $\quad -10$  & $3.84$\; \hspace{7pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (0.86,0.2);
    }   & $8.91$\; \hspace{6.5pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (1.55,0.2);
    } \\
  &    &  $\qquad \; 0$  & $2.95$\; \hspace{7pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (0.74,0.2);
    } & $3.57$\; \hspace{6.5pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.74,0.2);
    } \\
   &  &  $\qquad 10$  & $2.18$\; \hspace{7.5pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (0.63,0.2);
    }  & $0.82$\; \hspace{7pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.23,0.2);
    }\\
 &     &  $\qquad 20$  & $\mathbf{2.06}$ \hspace{7.5pt}  \tikz{
        \fill[fill=color4] (0.0,0) rectangle (0.60,0.2);
    } & $\mathbf{0.51}$ \hspace{7.5pt}  \tikz{
        \fill[fill=color9] (0.0,0) rectangle (0.19,0.2);
    } \\ \hline
 & \qquad $4$   &  $ \quad -10$ &  $2.82$ \hspace{9pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (0.7,0.2);
    }  & $2.61$\;\hspace{10pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (0.64,0.2);
    }  \\
  &    & $\qquad  0$  & $ 1.67$\hspace{12pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (0.55,0.2);
    }   & $0.87$\;\hspace{10.5pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.24,0.2);
    }\\
   &   & $\qquad 10$ & $1.23$\;\hspace{10pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (0.4,0.2);
     } & $0.41$\;\hspace{10.5pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.16,0.2);
     } \\
   & &  $\qquad 20$  & $\mathbf{1.03}$ \hspace{8pt}  \tikz{
        \fill[fill=color4] (0.0,0) rectangle (0.3,0.2);
    }  & $\mathbf{0.38}$ \hspace{8pt}  \tikz{
        \fill[fill=color9] (0.0,0) rectangle (0.14,0.2);
    }\\
&    & &     \ \ \ \ \ \ \ \ \hspace{-6pt} \qquad \tikz{
        \draw[black] (2.3,0) -- (5.2,0);
        \draw[black] (2.3,-2pt) -- (2.3,2pt)node[anchor=north] {\tiny$0$};
        \draw[black] (3.75,-2pt) -- (3.75,2pt)node[anchor=north] {\tiny$7.5$};
        \draw[black] (5.2,-2pt) -- (5.2,2pt)node[anchor=north] {\tiny$15$};
    } \vspace{0mm} &  \ \ \ \ \ \ \ \ \hspace{-6pt} \qquad \tikz{
        \draw[black] (2.3,0) -- (5.2,0);
        \draw[black] (2.3,-2pt) -- (2.3,2pt)node[anchor=north] {\tiny$0$};
        \draw[black] (3.75,-2pt) -- (3.75,2pt)node[anchor=north] {\tiny$7.5$};
        \draw[black] (5.2,-2pt) -- (5.2,2pt)node[anchor=north] {\tiny$15$};
    } \vspace{0mm} \\
    \bottomrule[1pt]
\end{tabularx}
\end{table*}


   \begin{table*}[t]
    \centering
    \caption{State and Action Prediction NRMSE for different latent state representation dimensions and training periods.} 
    \label{Table_3}
\begin{tabularx}{1\linewidth}{p{1.5cm} p{2cm} p{2.4cm} p{4cm} p{4cm}}
    \toprule[1pt]
    & Representation Dimension $d$ & Trajectory Length [s] & State Prediction NRMSE [\%] & Action Prediction NRMSE [\%]\\     
    \cmidrule(r){2-2} \cmidrule(r){3-3} \cmidrule(r){4-4}  \cmidrule(r){5-5}
 & $\qquad \quad 1$   &  $\qquad \quad 150$   & $10.71$\hspace{5pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (2.3,0.2);
    } & $1.54$\hspace{8pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (0.59,0.2);
    } \\
 &    & $\qquad \quad 250$  & $9.20$\hspace{9pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (2.01,0.2);
    } & $0.55$\hspace{8pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.21,0.2);
    } \\
  &    & $\qquad \quad 350$& $\textbf{7.99}$\hspace{9.75pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (1.77,0.2);
     } & $\textbf{0.29}$ \hspace{6.04pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.13,0.2);
    } \\ \hline
   & $\qquad \quad 2$ &  $\qquad \quad 150$  & $5.04$ \hspace{5.75pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (1.04,0.2);
    } & $1.54$ \hspace{5.5pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (0.59,0.2);
    }  \\
    &   &  $\qquad \quad 250$  & $4.93$ \hspace{5.75pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (0.97,0.2);
    } & $0.52$ \hspace{5.75pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.19,0.2);
    }\\
    & &  $\qquad \quad 350$  & $\textbf{3.73}$ \hspace{7.0pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (0.87,0.2);
    } & $\textbf{0.35}$ \hspace{6.75pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.16,0.2);
    }  \\ \hline
  & $\qquad \quad 3$ &  $\qquad \quad 150$  & $3.99$ \hspace{6.75pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (0.91,0.2);
    } & $1.51$ \hspace{5.75pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (0.58,0.2);
    } \\
   &  &  $\qquad \quad 250$  & $2.06$ \hspace{7pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (0.60,0.2);
    } & $0.51$ \hspace{6pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.19,0.2);
    } \\
    &  &  $\qquad \quad 350$  & $\textbf{1.22}$ \hspace{8pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (0.42,0.2);
    } & $\textbf{0.29}$ \hspace{7.5pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.13,0.2);
    } \\ \hline
    & $\qquad \quad 4$ &  $\qquad \quad 150$  & $1.28$ \hspace{7pt}  \tikz{
        \fill[fill=color1] (0.0,0) rectangle (0.48,0.2);
    } & $1.35$ \hspace{6.5pt}  \tikz{
        \fill[fill=color6] (0.0,0) rectangle (0.53,0.2);
    } \\
     & &  $\qquad \quad 250$  & $1.03$ \hspace{7pt}  \tikz{
        \fill[fill=color2] (0.0,0) rectangle (0.3,0.2);
    } & $0.38$ \hspace{6.75pt}  \tikz{
        \fill[fill=color7] (0.0,0) rectangle (0.14,0.2);
    } \\
     & &  $\qquad \quad 350$  & $\textbf{0.96}$ \hspace{8pt}  \tikz{
        \fill[fill=color3] (0.0,0) rectangle (0.29,0.2);
    } & $\textbf{0.22}$ \hspace{8pt}  \tikz{
        \fill[fill=color8] (0.0,0) rectangle (0.10,0.2);
    } \\
     
 &    & &\ \ \ \ \ \ \ \ \hspace{-9pt} \qquad \tikz{
        \draw[black] (2.3,0) -- (5.2,0);
        \draw[black] (2.3,-2pt) -- (2.3,2pt)node[anchor=north] {\tiny$0$};
        \draw[black] (3.75,-2pt) -- (3.75,2pt)node[anchor=north] {\tiny$7.5$};
        \draw[black] (5.2,-2pt) -- (5.2,2pt)node[anchor=north] {\tiny$15$};
    } \vspace{0mm} &\ \ \ \ \ \ \ \ \hspace{-9pt} \qquad \tikz{
         \draw[black] (2.3,0) -- (5.2,0);
        \draw[black] (2.3,-2pt) -- (2.3,2pt)node[anchor=north] {\tiny$0$};
        \draw[black] (3.75,-2pt) -- (3.75,2pt)node[anchor=north] {\tiny$7.5$};
        \draw[black] (5.2,-2pt) -- (5.2,2pt)node[anchor=north] {\tiny$15$};
    } \vspace{0mm} \\
    \bottomrule[1pt]
\end{tabularx}
\end{table*}

 \vspace{3pt}\noindent\textbf{Prediction accuracy:}\, Since the main goal of the proposed sensing Koopman AE and the controlling Koopman AE is to predict future system states and control action commands, respectively, we use the normalized root mean square error $\left( \mathrm{NRMSE}\right)$ to evaluate the quality of prediction performance. The $\mathrm{NRMSE}$ is the root mean squared error between the predicted and observed signals in a prediction window of length $M_{p}$ normalized by the norm of the difference between the minimum and maximum vectors of the observed signals, \begin{align}
     \label{eq_RMSE_state}
     \mathrm{NRMSE}_{M_{p}} = \frac{ \sqrt{ \frac{1}{M_{p}} \sum_{ m  = M_{\scriptscriptstyle \text{s}+1} }^{M_{\scriptscriptstyle \text{s}} + M_{p}}  \| \bar{\mathbf{x}}_{m} - \hat{\mathbf{x}}_{m} \|_{2}^2 }} { \| \max (\hat{\mathbf{x}}) -  \min (\hat{\mathbf{x}}) \|_{2}} \times 100,
     \end{align}where $M_{p}$ is the prediction time horizon at test that the remote controller makes in the second phase of the remote controlling. Note that if the second phase becomes long, there will be error propagation that will degenerate the prediction performance. As a result, we have two options to enhance the prediction performance: 1) sending a new latent state representation to initialize the prediction, and 2) shifting to the first phase of remote controlling to fine-tune the trained Koopman operator. 
 
 
 \vspace{3pt}\noindent\textbf{Wireless communication metric:}\, To validate the performance of the proposed Koopman AE in terms of communication efficiency, we measure the maximum number of consecutive lost packets $M_{\text{lost}}$ until the most recent successful transmission. Hence, the number of consecutive lost packets linearly increases with time if the transmitter-receiver pair experiences adverse channel conditions or the prediction accuracy of the Koopman AE reaches a predefined threshold.     
 
 \vspace{3pt}\noindent\textbf{Control stability:}\, is a control performance metric in terms of the control system response to any initial condition. The control system is said to be asymptotically stable if, for  every $\epsilon > 0$, $m \geq 0 $, and a given control action command, there exists $\| \mathbf{x}_{m} - \mathbf{x}_{d} \|^{2}_{2} < \epsilon$ as $ m \rightarrow \infty$, where $\mathbf{x}_{d} \in \mathbb{R}^{p}$ is the desired system state~\cite{hangos2004analysis}. Then, the control stability along the prediction time horizon at test is the mean squared control error, i.e., the time-averaged of squared system states deviation from its desired state along the prediction time horizon at the test, given as \begin{align}
     \label{eq_MSCE}
     \mathrm{MSCE}_{M_{p}} =  \frac{1}{M_{p}} \sum_{m=1}^{M_{p}}  \| \mathbf{x}_{m} - \mathbf{x}_{d} \|_{2}^{2}.
 \end{align} Note that the control stability in the proposed approach depends on the prediction accuracy that are affected by the communication efficiency, highlighting the importance of jointly designing communication, learning, and control operations.

 \begin{figure*}
    \centering
    \subfigure[]{\includegraphics[width=0.4\textwidth]{Fig/Training_loss_5.eps}} 
    \subfigure[]{\includegraphics[width=0.4\textwidth]{Fig/Training_q_3.eps}} 
    \caption{Training loss of the sensing Koopman AE with (a) different SNR and (b) different latent state representation dimensions. }
    \label{fig Train_Loss}
  \end{figure*} 

  \subsection{Performance Evaluation of Split Koopman AE}
  \label{Performance_Evaluation}
  In this subsection, we evaluate the performance of the proposed two-way split Koopman AE for different communication, prediction, and control parameters.    

   \vspace{3pt}\noindent\textbf{SNR  Vs. State Prediction Accuracy.}\quad Fig.~\ref{fig state_prediction} demonstrates the prediction performance of the proposed sensing Koopman AE compared to the non-predictive remote monitoring of the non-linear inverted cart-pole system. The remote controller in the proposed sensing Koopman AE predicts the future time-series system states with different SNR and one-step target prediction depth considered in training compared to the remote controller in the non-predictive remote monitoring that receives the non-linear system states at each time slot over an ideal channel. It can be seen that the predicted system states of the proposed sensing Koopman AE with high SNR, i.e., $\text{SNR} \in \{10,20\}$ $\mathrm{dBm}$  match closely the observed system states in the non-predictive remote monitoring compared to the predicted system states with low SNR, i.e., $\text{SNR} \in \{-10,0\}$ $\mathrm{dBm}$.      
   
   The reason behind this result is that the stability of training the sensing Koopman AE relies on the communication reliability of the observed system states at the remote controller, highlighting the importance of co-designing the communication and deep learning operations. As a result, the state prediction accuracy is improved at the cost of increasing communication resources in terms of transmission power and allocated channel bandwidth. Moreover, the state prediction results in Fig.~\ref{fig state_prediction} emphasize the ability of the sensing Koopman AE in discovering the Koopman invariant subspace with four latent state representations and one-step target prediction depth considered in training. Then, the sensing Koopman AE globally linearizes the non-linear system dynamics of the inverted cart-pole and predicts the future system states at the remote controller based on the trained Koopman matrix, improving the forward link communication efficiency.           
   

   
   \vspace{3pt}\noindent\textbf{SNR  Vs. Action Prediction  Accuracy.}\quad  For the proposed controlling Koopman AE depicted in Fig.~\ref{fig_force}, the actuator predicts the future control action commands with different SNR values, and one-step target prediction depth considered in training compared to the actuator in the non-predictive remote controlling of the non-linear inverted cart-pole system that observes the control action commands calculated over Jacobian linearization method at each time slot over an ideal channel. Here, the transmission power in both the forward and reverse communications are linked together since the observed control action command at the actuator is based on the observed system states affecting the control action prediction performance and the control stability. It is clear that the predicted control action commands in the controlling Koopman AE with high SNR, i.e., $\text{SNR} \in \{10,20\}$ $\mathrm{dBm}$ approximately coincides with the observed control action commands compared to the predicted control action commands with low SNR, $\text{SNR} \in \{-10,0\}$ $\mathrm{dBm}$.  
   
   
   The rationale behind this result is that the learning stability of the controlling Koopman AE depends on the communication reliability of the observed control action commands at the actuator, highlighting the importance of jointly designing the communication, learning, and control operations. Hence, the action prediction accuracy is improved which yields stabilized control system at the expense of utilizing high communication resources in terms of transmission power and allocated channel bandwidth in the first phase of remote controlling. Moreover, the action prediction results in Fig.~\ref{fig_force} depict the ability of the controlling Koopman AE in capturing the non-linear action dynamics. Hence, the controlling Koopman AE  has the ability to predict the future control action commands, improving both the forward and reverse links communication efficiency.   
   
 \begin{figure*}
    \centering
    \subfigure[State prediction performance.\label{fig_pred_depth_a}]{\includegraphics[width=0.4\textwidth]{Fig/State_Pred_Vs_Pred_Iinterval_5.eps}} 
    \subfigure[State training completion time.\label{fig_pred_depth_b}]{\includegraphics[width=0.4\textwidth]{Fig/State_Comp_Time_2.eps}}
    \subfigure[Action prediction performance.\label{fig_pred_depth_c}]{\includegraphics[width=0.4\textwidth]{Fig/State_Comp_Time_3.eps}} 
    \subfigure[Action training completion time.\label{fig_pred_depth_d}]{\includegraphics[width=0.4\textwidth]{Fig/Control_Comp_Time_2.eps}} 
    \caption{Prediction performance and training completion time of both the proposed split sensing Koopman learning and the proposed split controlling closed-loop Koopman learning for different target prediction depths and different SNR values.}
    \label{fig_pred_depth}
  \end{figure*}
 
   \vspace{3pt}\noindent\textbf{SNR  \& Representation Dim Vs. Prediction Accuracy.}\quad As shown in Fig.~\ref{fig state_prediction}, the state prediction performance of the sensing Koopman AE is improved at the cost of increasing the communication resources in terms of four-dimensional latent state representations and a high SNR value. Table~\ref{Table_1} describes the state prediction performance of the sensing Koopman AE for different SNR values and different latent state representation dimensions. From this table, it is clear that the state prediction accuracy is improved at the cost of increasing the SNR for the same latent state representation dimension, the same sensor transmission power, the same distance from the sensor to the controller, one-step target prediction depth considered in training, and the same training period. The state prediction accuracy is almost the same in the lowest latent state representation dimension, i.e., $d = 1$, for low SNR values, i.e., $\text{SNR} \in \{-10,0,10\}$ dBm. In contrast, the state prediction accuracy is improved by increasing the SNR values in the other latent state representation dimensions $d \in \{2,3,4\}$. The rationale behind the state prediction results in Table~\ref{Table_1} is that the lowest latent state representation dimension is not enough to discover the Koopman invariant subspace in the observables space of the non-linear inverted cart-pole system affecting the state prediction performance. Hence, for obtaining high state prediction performance, the linearized Koopman subspace reflecting the non-linear system dynamics is obtained at the expense of increasing the communication resources in terms of selecting a high SNR value and a large latent state representation dimension, leading to a trade-off between the communication cost and the prediction accuracy.  
   
   
   Table.~\ref{Table_1} demonstrates also the control action prediction performance of the controlling Koopman AE compared to the non-predictive remote controlling of the non-linear inverted cart-pole system. The controlling Koopman AE located at the actuator locally predicts the future control action commands for different SNR values and different latent state representation dimensions. Note that the control action prediction performance is improved at the cost of increasing the SNR value for the same latent state representation dimension, the same controller transmission power, the same distance from the controller to the actuator, one-step target prediction depth considered in training, and the same training period. Additionally, for the same SNR value, we notice that the control action prediction performance is almost the same for the low latent state representation dimensions of $d  \in \{1,2,3 \} $ compared to the four-dimensional latent state representation. This demonstrates the trade-off between the communication payload size and the control action prediction accuracy, in addition to the fact that the four-dimensional latent state representations quickly improve the control action prediction accuracy as a result of reflecting the non-linear action dynamics in the controlling Koopman invariant subspace.
  
  \vspace{3pt}\noindent\textbf{Trajectory Length \& Representation Dim Vs. Prediction Accuracy.}\quad As a result of the difficulty in identifying the non-linear dynamics in an interpretable way, the controller in the non-predictive remote controlling case receives the system states at each time slot and calculates the control action using the non-linear control theory. In contrast, our proposed sensing Koopman AE identifies the non-linear system dynamics in an interpretable linear form that is utilized by the remote controller to calculate the optimal control action using the linear control theory and to predict the future system states even without communication. Table.~\ref{Table_3} demonstrates the state prediction accuracy of the sensing Koopman AE for the same sensor transmission power, the same distance from the sensor to controller, different training periods, different latent state representation dimensions, and one-step target prediction depth considered in training. The state prediction accuracy is improved as the training period increases for the same SNR value and the same latent state representation dimensions, highlighting the trade-off between the state prediction accuracy and the communication payload size. The state prediction accuracy in Table~\ref{Table_3} is improved as a result of increasing the number of observed system states per trajectory for the same SNR value and the same latent state representation dimension. The rationale behind this result is that increasing the number of observed system states per trajectory ensures the training dataset is rich enough to represent the non-linear system dynamics and guarantees the robustness of discovering the Koopman invariant subspace at the expense of increasing the communication resources.       
  
  \begin{figure*}[t!]
    \centering
    \subfigure[State prediction performance. \label{fig_state_repesentations_a}]{\includegraphics[width=0.4\textwidth]{Fig/State_Pred_Repres_6.eps}} 
    \subfigure[ State training completion  time.\label{fig_state_repesentations_b}]{\includegraphics[width=0.4\textwidth]{Fig/State_Pred_Repres_Time_1.eps}} 
    \caption{Prediction performance and training completion time of the proposed sensing Koopman AE with a ten-step target prediction depth, different latent state representation dimensions $ d \in \{ 4, 6, 8, 10, 12, 14\} $, and  $\mathrm{SNR} = 20 \, \mathrm{dBm}$.}
    \label{fig_state_repesentations}
  \end{figure*}  
  
  Table.~\ref{Table_3} demonstrates also the control action prediction performance of the controlling Koopman AE for the same controller transmission power, the same distance from the sensor to controller, different training periods, different latent state representation dimensions, and one-step target prediction depth considered in training. It is clear that the control action prediction performance is improved at the cost of increasing the number of received control action commands per trajectory in the training dataset for the same SNR value and the same latent state representation dimension, highlighting the trade-off between the action prediction performance and the communication payload size. Moreover, the action prediction performance is almost the same for low latent state representation dimensions $d \in \{1,2,3\} $, the same target SNR, and the same trajectory length compared to the action prediction performance for the four-dimensional latent state representation. The reason behind this result is that the low latent state representation dimensions are insufficient to discover the controlling Koopman invariant subspace of the non-linear action dynamics. Additionally, for the same latent state representation dimension, increasing the trajectory length increases the action prediction performance since the high sampling rate helps in describing the non-linear action dynamics and discovering the controlling Koopman invariant subspace.
  
  
  \vspace{3pt}\noindent\textbf{SNR \& Representation Dimensions vs. Training Loss.}\quad Fig.~\ref{fig Train_Loss} demonstrates the overall training loss of the sensing Koopman AE for different SNR values and different latent state representation dimensions. For the same latent state representation dimension, i.e., $d= 3$, it is clear that the training loss with the lowest SNR value, i.e., $\mathrm{SNR} = -10$ $\mathrm{dBm}$ converges faster compared to the other SNR values at the cost of achieving low training accuracy. In contrast, the training loss with the high SNR, i.e., $\mathrm{SNR} = 20$ $\mathrm{dBm}$ converges slowly to the minimum value compared to the other SNR values, i.e., $\text{SNR} \in \{-10, 0, 10\}$ $\mathrm{dBm}$.  This in turn shows the impact of the SNR value on the training accuracy in which the received data samples to the another part of the sensing Koopman AE affects the training accuracy, convergence speed, and communication payload size.    
 
  For the same SNR value, we can see that the training loss of the sensing Koopman AE slowly converges as the representation dimension increases. More specifically, the communication payload size of the forward and backward propagation signals is proportional to the number of weights parameters in the Koopman hidden layer. As a result, increasing the latent state representation dimensions results in a high latency for transmitting the forward and backward propagation signals which leads to high prediction accuracy, highlighting the trade-off between the prediction accuracy, transmission latency, and communication payload size.
  
 \begin{figure*}[t!]
    \centering
    \subfigure[State prediction performance.\label{fig_state_traj_a}]{\includegraphics[width=0.4\textwidth]{Fig/State_Pred_Traj_3.eps}} 
    \subfigure[State training completion time. \label{fig_state_traj_b}]{\includegraphics[width=0.4\textwidth]{Fig/State_Pred_Traj_Time_1.eps}} 
    \subfigure[Action prediction performance. \label{fig_state_traj_c}]{\includegraphics[width=0.4\textwidth]{Fig/Control_Pred_Traj_3.eps}} 
    \subfigure[Action training completion time. \label{fig_state_traj_d}]{\includegraphics[width=0.4\textwidth]{Fig/Control_Pred_Traj_Time_1.eps}} 
    \caption{Prediction performance and training completion time of the proposed sensing Koopman AE with a one-step target prediction depth, different number of trajectories in the training dataset $T_{t} = \{ 70, 700 \} $, different SNR values $\mathrm{SNR} = \{ 20, 0, -10  \} \, \mathrm{dBm}$. }
    \label{fig_state_traj}
  \end{figure*} 
 
  
 \vspace{3pt}\noindent\textbf{Target Prediction Depth Vs.  Prediction Performance \& Training Completion Time.}\quad To dive deeper into the benefits of both the sensing Koopman AE and the controlling Koopman AE, we increase the range of random initial conditions to generate the training dataset as $[-2.0,2.0]$ for each state dimension and also increase the trajectory length as $\mathcal{M}_{\mathrm{Train}} = 500 \, \mathrm{s}$. Here, the results are obtained based on averaging several training runs with different seeds. Fig.~\ref{fig_pred_depth_a} and Fig.~\ref{fig_pred_depth_c} show the prediction performance of the sensing Koopman AE and the controlling Koopman AE, respectively for different target prediction depths considered in training, different SNR values, and four-dimensional latent state representations. For the same target prediction depth considered in training, we can see that the state prediction performance decreases as the prediction time horizon at the test increases due to the error propagation as the prediction time increases. As a result, based on a predefined prediction threshold, we send a new latent state representation or shift to the first phase of remote control to enhance the state prediction performance.

 For the same SNR value, it is clear that the prediction performance of the split Koopman AE with a one-step target prediction depth considered in training is better than that with a ten-step target prediction depth over different prediction time horizons at the test time, i.e., increasing the target prediction depth deteriorates the prediction performance over different prediction time horizons at the test. The rationale behind this result is that the small errors in training the Koopman operator with a high target prediction depth during the first phase of remote control lead to large errors when evaluating the prediction performance for a large prediction time horizon at the test.   
 
 Fig.~\ref{fig_pred_depth_b} and Fig.~\ref{fig_pred_depth_d} show the training completion time required to train the sensing Koopman AE and the controlling Koopman AE, respectively, for different SNR values and different target prediction depths. For the same SNR value, it is clear that the training completion time associated with a ten-step target prediction depth is larger than that with a one-step target prediction depth due to the high computational complexity associated with a ten-step target prediction depth considered in training. Hence, increasing the target prediction depth considered in training leads to a high training completion time and a high communication payload size due to the necessity to transmit the system states in the first phase of remote control until the sensing Koopman AE is well-trained. 


 By analyzing both the prediction performance and the training completion time of the split Koopman AE, we can see that the split Koopman AE with one-step target prediction depth and a low SNR value has better prediction performance compared to that with ten-step target prediction and a high SNR value. In addition, the split Koopman AE with one-step target prediction depth has a low communication cost in terms of transmission power and communication payload size. For instance, the split Koopman AE with one-step target prediction depth and $\mathrm{SNR} = 0 \, \mathrm{dBm}$ has better prediction performance compared to that with ten-step target prediction depth and $\mathrm{SNR} = 20 \, \mathrm{dBm}$. Overall, increasing the target prediction depth with the current hyperparameter setting deteriorates the prediction performance compared to the low target prediction depth. Hence, we next study the effect of changing the latent state representation dimensions on the prediction performance with a ten-step target prediction depth for the same SNR value. 
 
 
 \vspace{3pt}\noindent\textbf{Representation Dim Vs. Prediction Performance \& Training Completion Time.}\quad Fig.~\ref{fig_state_repesentations} presents the prediction performance and training completion time of the sensing Koopman AE for different latent state representation dimensions, ten-step target prediction depth considered in training, $\mathrm{SNR} = 20 \, \mathrm{dBm}$, and the same previous hyperparameter setting. First, it is clear from Fig.~\ref{fig_state_repesentations_a} that the prediction performance of the sensing Koopman AE with a ten-step target prediction depth is improved at the cost of increasing the latent state representation dimensions, highlighting the trade-off between the target prediction depth considered in training and the latent state representation dimensions. Furthermore, we can see that the prediction performance with a ten-step target prediction depth starts to saturate after twelve-dimensional latent state representations over different prediction time horizons at the test. The reason behind this result is that increasing the latent state representation dimensions in the high target prediction depth setting ensures discovering the Koopman invariant subspace that guarantees high prediction performance for a long prediction time horizon at the test. Hence, selecting a large dimension of latent state representations with a large target prediction depth is instrumental in casting non-linear system dynamics in a linear form at the expense of increasing the communication payload size, leading to a trade-off between the communication cost and the prediction performance with a high target prediction depth considered in training.   
 
 Fig.~\ref{fig_state_repesentations_b} shows the training completion time required to train the sensing Koopman AE with a ten-step target prediction depth considered in training and different latent state representation dimensions. We can see that the training completion time increases as the latent state representation dimensions increase until eight-dimensional latent state representations, after which it starts to decrease until twelve latent state representation dimensions, then it is almost the same. The reason behind this result is that increasing the latent state representation dimensions in the large target prediction depth considered in training hastens the convergence speed of the sensing Koopman AE training to discover the Koopman invariant subspace. As a result, reducing the communication payload size required to observe the system states in the first phase of remote control until the sensing Koopman AE is well trained.
 
  
 \vspace{3pt}\noindent\textbf{Trajectories Number Vs.  Prediction Performance \& Training Completion Time.}\quad Fig.~\ref{fig_state_traj_a} and Fig.~\ref{fig_state_traj_c} demonstrate the prediction performance of the sensing Koopman AE and the controlling Koopman AE, respectively, with a one-step target prediction depth considered in training, four-dimensional latent state representations, the same previous hyperparameter setting,  different SNR values, and a different number of trajectories in the training dataset. For the same SNR value, it is clear that the prediction performance of the split Koopman AE is improved over different prediction time horizons at the test by increasing the number of trajectories in the training dataset as a result of well representing the non-linear system dynamics by increasing the number of trajectories in the training dataset. For the same number of trajectories, we can see the impact of the SNR on the prediction performance, in which the prediction performance with a high SNR value is higher than that with a low SNR value. For example, the controlling Koopman AE with $T_{t} = 700$ and $\mathrm{SNR} = 20 \, \mathrm{dBm}$ has higher prediction performance compared to that with the other SNR values, i.e., $\mathrm{SNR} \in \{0, -10 \} \, \mathrm{dBm}$. In addition, the controlling Koopman AE with $T_{t} = 70$ and $\mathrm{SNR} = 20 \mathrm{dBm}$ has almost the same prediction performance compared to that with $T_{t} = 700$ and $\mathrm{SNR} = 0 \, \mathrm{dBm}$ while it has better prediction performance compared to the others with different number of trajectories and low SNR values. This presents the relationship between the SNR value and the number of trajectories in the training dataset, in which a large number of trajectories in the training dataset with a high SNR value has a much larger prediction performance compared to those that have the same number of trajectories with low SNR values. Otherwise, choosing a low number of trajectories in the training dataset with a high SNR value has better prediction performance compared to those with a large number of trajectories in the training dataset with a low SNR value, highlighting the trade-off between the communication payload size and the SNR value in improving the prediction performance.
 

 Fig.\ref{fig_state_traj_b} and Fig.~\ref{fig_state_traj_d} show the training completion time required to train the sensing Koopman AE and the controlling Koopman AE, respectively for a different number of trajectories in the training dataset, different SNR values, and the same hyperparameter setting. For the same SNR value, it is clear that the training completion time increases as the number of trajectories in the training dataset increases as a result of increasing the payload size of the forward and backward propagation signals to train the split Koopman AE. For the same number of trajectories in the training dataset, it is clear that the training completion time of the split Koopman AE with a large number of trajectories in the training dataset decreases as the SNR value increases. The reason behind this result is that observations received at another part of the split Koopman AE are sufficient and reliable to discover the Koopman invariant subspace. In contrast, decreasing the SNR value for the same large number of trajectories in the training dataset increases the training completion time, leading to a trade-off between the training completion time and the communication cost in terms of the SNR value and the number of trajectories in the training dataset.
  
 \begin{figure}
 \centering
 \includegraphics[ width=0.4\textwidth]{Fig/MSCE_Vs_Number_2.eps} \\
 \caption{Control stability for the split Koopman AE and the non-predictive remote controlling over different values of consecutive packet losses with different SNR values.} \label{fig_MSCE}
 \end{figure}
 
 \begin{figure*}[t!]
    \centering
    \subfigure[Cart position.]{\includegraphics[width=0.4\textwidth]{Fig/Jacob_Position_1.eps}} 
    \subfigure[Cart velocity]{\includegraphics[width=0.4\textwidth]{Fig/Jacob_Velocity_1.eps}} 
    \subfigure[Pendulum angular position.]{\includegraphics[width=0.4\textwidth]{Fig/Jacob_Pend_1.eps}} 
    \subfigure[Pendulum angular velocity.]{\includegraphics[width=0.4\textwidth]{Fig/Jacob_Pend_Vel.eps}} 
    \caption{Comparison of Koopman-based Controller versus Jacobian-based Controller (a) Cart Position (b) Cart Velocity (c) Pendulum angular position and (d) Pendulum angular velocity. }
    \label{fig_Controller}
\end{figure*}   
   
 \vspace{3pt}\noindent\textbf{Control Stability Vs. Consecutive Packet Losses.}\quad Fig.~\ref{fig_MSCE} illustrates the control stability, i.e., the mean squared control error, over different values of consecutive packet losses with different SNR values. It is clear that the mean squared control error for the split Koopman AE is almost the same as the number of consecutive packet losses increases compared to the non-predictive remote control. The rationale behind this result is that the sensing Koopman AE at the remote controller compensates for the missing system states by locally predicting them after observing a sufficient number of system states along with their latent state representations over favorable channel conditions with different SNR values. Moreover, the actuator locally predicts the missing control action commands utilizing the trained controlling Koopman AE after observing a sufficient number of control action commands, thereby improving the communication efficiency and the control performance. The control performance of the proposed split Koopman AE with $\mathrm{SNR} = 0 \, \mathrm{dBm}$ is less than that of one with $\mathrm{SNR} = 20 \, \mathrm{dBm}$ as a result of the communication reliability impact on the prediction accuracy. 
 
 


 \vspace{3pt}\noindent \textbf{Koopman-based Vs. Jacobian-based Linear Controller} In Fig.~\ref{fig_Controller}, we show the inverted cart-pole system states for the Koopman-based controller and Jacobian-based controller. Here, the inverted cart-pole system is assumed to be operated from an initial condition far from the equilibrium point, i.e., $\mathbf{x}_{0} = [2.5 \; 2.5 \; 2.5 \; 2.5 ]^{\mathsf{T}}$. Note that the Koopman-based linear controller drives the inverted cart-pole system to the desired states compared to the Jacobian-based controller. The rationale behind failing the Jacobian-based controller in stabilizing the non-linear system is that the initial condition is far from the equilibrium point, $\mathbf{x}_{d} = [0 \; 0 \; 0 \; 0 ]^{\mathsf{T}}$ compared to the Koopman-based linear controller that is robust against the initial condition as a result of obtaining a linearized Koopman invariant subspace reflecting the non-linear dynamics with high accuracy.    
 

 
 
 
 
